Assessing the impact of transient orbital resonances

One of the primary sources for the future space-based gravitational wave detector, the Laser Interferometer Space Antenna, are the inspirals of small compact objects into massive black holes in the centres of galaxies. The gravitational waveforms from such Extreme Mass Ratio Inspiral (EMRI) systems will provide measurements of their parameters with unprecedented precision, but only if the waveforms are accurately modeled. Here we explore the impact of transient orbital resonances which occur when the ratio of radial and polar frequencies is a rational number. We introduce a new Effective Resonance Model, which is an extension of the numerical kludge EMRI waveform approximation to include the effect of resonances, and use it to explore the impact of resonances on EMRI parameter estimation. For one-year inspirals, we find that the few cycle dephasings induced by 3:2 resonances can lead to systematic errors in parameter estimates, that are up to several times the typical measurement precision of the parameters. The bias is greatest for 3:2 resonances that occur closer to the central black hole. By regarding them as unknown model parameters, we further show that observations will be able to constrain the size of the changes in the orbital parameters across the resonance to a relative precision of 10% for a typical one-year EMRI observation with signal-to-noise ratio of 20. Such measurements can be regarded as tests of fundamental physics, by comparing the measured changes to those predicted in general relativity.

==> referee_response.tex <==
To the Editors,

We thank the referee for the very useful report. We have carefully worked through the suggestions and comments, itemized below, and made revisions to the text as noted. We hope that the manuscript now addresses all concerns and questions, and is suitable for publication.

Sincerely,

L. Speri 
J. Gair

----------------------------------------------------------------------
Report of the Referee -- DC12964/Speri
----------------------------------------------------------------------

1) In Section I, paragraph 6 (page 2), I recommend that the authors provide citations when first introducing the gravitational self-force. I would recommend the original papers by Mino, Sasaki, and Tanaka (1997), and Quinn and Wald (1997).

We provided the requested citations (now number 38,39).

2) In Section IIB, paragraph 2 (page 3), I recommend that the authors reference the works that first introduced the angle parameterization used in Eq (4), which I believe are Schmidt (2002) (which the authors reference at another point as Ref [47]), and Drasco and Hughes (2004).

We provided the requested citations (now number 59,63).

3) In Section IIC (page 5), there are a couple of errors in Eq (9). Both inner products contain double vertical bars instead of the single
vertical bars that the authors used in previous notation. Additionally, there are two plus signs back-to-back (at the end of the first line and beginning of the second). These will need to be
corrected.

We thank the referee for pointing this out. We corrected the plus signs. The double vertical bars were a rendering problem, but we hope we have fixed this by using a different set of latex commands.

4) In Section IIIB (page 7), I believe there is an error in the second sentence following Eq (12). The authors' inline equation for $\xi$ does not match any of the previous or following definitions for $\xi$. If this is not an error, then I recommend that the authors elaborate on why the definition of $\xi$ has changed here.

Again, we thank the referee for spotting this error. We corrected the inline equation.

5) In Section IIIC, paragraph 1, sentence 2 (page 7), the authors state, "The value of $\mathcal{C}$ for a specific trajectory can be determined by calculating the full, oscillatory term $G$ following the procedure described in [59]. However, this requires a full GSF calculation for a generic EMRI inspiral..." Did the authors mean to use a different reference here? Reference [59] details a procedure for calculating parts of G (i.e., the pieces of G that appear in Eq (11) of this paper), but it does not give a procedure for calculating the full oscillatory part of G, nor the GSF. In fact, [59] explicitly avoids calculating the GSF. If this is the reference that the authors meant to use here, then these sentences need to be rewritten to more accurately reflect the results of [59].

We definitely used the wrong words to reflect the work done in Flanagan 2014 (old ref[59], new ref[47]). We rephrased the sentence as follows:
"The value of $\mathcal{C}$ for a specific trajectory can be estimated by using Eq.(11) following the procedure described in ref [47].
However, this procedure is currently too computationally expensive for our purposes.".

6) In Section IVA, paragraph 2 (page 9), the authors state, "Previous investigations have considered a limited set of EMRI configurations and analysed the dephasings induced by resonances using a Post-Newtonian model for the resonant force [37, 59]." Again, I think [59] is mis-referenced here. Reference [59] does not use a Post-Newtonian model. Possibly the authors meant to reference [36] instead, which does explore EMRI resonances with Post-Newtonian results.

We mis-referenced the work from Flanagan 2014. We wanted to reference Flanagan 2012 (now ref[40]) and Berry (2016) (now ref[41]) where they used Post-Newtonian models.

7) In Section IVA, paragraph 3 (page 9), I recommend that the authors rewrite part of the discussion concerning the impact of "inclination."
I found the authors' use of "inclination" confusing. For example, consider the statement, "The dephasings increase with decreasing
inclination...". When the authors say "inclination" do they mean inclination with respect to the orbital plane? If so, then the inclination peaks at $\pi/2$, where the dephasing also appears to peak
in Figure 2. In that case, it looks like the dephasings decrease as one decreases inclination (i.e, as one moves closer to the equatorial
plane). If instead "inclination" refers to the inclination angle parameter $\iota$ (which is what I think the authors mean in this section), then this statement is supported by Figure 2 for retrograde orbits, but it remains unclear whether or not this statement is true for prograde orbits, because the authors do not plot inclinations
below $\iota = 1.3$ in Figure 2. Additionally, the authors state at the bottom of page 9, "the biggest phase shifts are for systems with low inclinations. These latter systems have resonances which occur closer to the central black hole...This leads to a higher $\Delta J(\tau_\mathrm{res}+\tau_\mathrm{start})$ compared to other configurations, and, as a consequence, higher phase shifts...as we can see from Figure (2)." If I look at Figure 2, the lowest inclination I see is $\iota = 1.3$, which is still an inclination of >70 degrees with respect to the orbital plane. I think most readers would consider
this to be a relatively large inclination. So this statement that low inclination orbits lead to higher phase shifts is confusing, and is
not fully supported by Figure 2. I would recommend that the authors be more explicit about what they mean by inclination (e.g., state "The
dephasings increase with decreasing $\iota$..."), and if the authors are going to discuss the dephasing behavior at "low inclinations,"
then the authors need to include low inclination data in Figure 2, or some other format that supports their claims. In fact, I believe this
discussion would be greatly aided if the authors plotted the dephasing for low values of $\iota$, since the authors claim that they performed
dephasing calculations for systems with inclination angles ranging from $ 0.1 <= \iota <= 3.1$.

We thank the referee for pointing this out and we are sorry for using the misleading term "inclination" to refer to the inclination angle parameter $\iota$. We replaced, where possible, the term inclination with $\iota$.

In the previous version we excluded the dephasings for $\iota<1.3$ because those systems have an inspiral shorter than one year. The dephasings were calculated for a fixed one-year duration and therefore adding data for $\iota<1.3$ would have not given a fair comparison.
However, we decided to update the figure with the dephasing calculations for systems with inclination angles ranging from $ 0.1 <= \iota <= 3.1$, as suggested by the referee, and we expanded the explanation in the section to explain the new features.


8) In Section IVC (page 10), Eq (15) there is another error where two vertical bars are used in the inner product.

As above. this appears to have been a pdf rendering problem which we hope is now fixed.

9) In Section V, paragraph 5 (page 13), the authors state, "The EMRI systems which are most affected by resonances provide measurements of the resonance coefficients with a relative precision ranging from 0.05
- 0.3 (median values)." These values do not match the values reported in the previous section (Sec IVD, paragraph 6), which range from 0.07
- 0.68. This may be a small typographic error or these results are being reinterpreted in Section V. If the latter is true, then I recommend that the authors expand upon why these values differ from the results reported in Sec IVD.

We thank again the referee, this was an error. We corrected the ranges.

We thank the referee for the optional suggestions. We found them extremely useful.

(OPTIONAL) SUGGESTIONS

1) There are just a handful of grammatical errors I found throughout
the paper that should be easy to fix:

- Section I, paragraph 2 (page 1), sentence 1: "ripples in the fabric
of spacetime allows us" ->  "ripples in the fabric of spacetime allow
us"

DONE

- Section IIA (page 2), there is a missing indent at the beginning of
paragraph 2

DONE

- Section IIA (page 3), there is a missing indent at the beginning of
paragraph 4

DONE

- Section III, paragraph 1, sentence 3 (page 5): "Flanaghan" ->
"Flanagan"

DONE

- Section III, paragraph 1, sentence 7 (page 5): "it is necessary to
build a model that take them into account" ->  "it is necessary to
build a model that takes them into account"

DONE

- Section IIIA, paragraph 3, sentence 3 (page 6): "an analogously for
the fundamental frequencies" ->  "and analogously for the fundamental
frequencies"

DONE

- Section IIIC, paragraph 2, sentence 2 (page 7): "Flanaghan" ->
"Flanagan"

DONE 

- Section IIID (page 8), there is either a missing indent at the
beginning of paragraph 2 or a misplaced line break following list
(i)-(iv) in paragraph 1

DONE

- Figure 5, sentence 2 (page 12): "measurement precision over randomly
draws" ->  "measurement precision over random draws"

DONE
 
2) In Section I, paragraph 3 (page 1), I recommend citing one of the
LISA white papers or LISA website, e.g. Amaro-Seoane (2017)

DONE

3) In Section I, paragraph 7 (page 2), among the references included
at the end of the sentence "EMRI resonances have been studied in a
number of previous works [38-42]", I recommend also including Hirata
(2011); Grossman, Levin, and Perez-Giz (2013); Flanagan, Hughes, and
Ruangsri (2014) (which the authors reference at another point as Ref
[59]); Ruangsri and Hughes (2014) (which the authors reference at
another point as Ref [58]); and Isoyama et al. (2019)

DONE

4) In Section I, paragraph 8 (page 2), recommend adding a reference
after the authors first introduce the Numerical Kludge model.

DONE

5) In Section IIA, paragraph 2 (page 3), the authors refer to $a$ as
the "dimensionless spin parameter," but $a$ is not dimensionless in Eq
(1), but $a/M$ is. I recommend that the authors just refer to $a$ as
"the Kerr spin parameter" or simply "the spin parameter." Or if they
want $a$ to be dimensionless, then I recommend that the authors
correct Eq (1) so that $a$ is dimensionless. Otherwise, latter
instances of $a$ will need to be corrected to $a/M$ in the paper
(e.g., the caption of Figure 1, the colorbar of Figure 2, the legend
and caption of Figure 3, the legend of Figure 4, the legend of Figure
5, as well as paragraph 4 of Section IVA and paragraph 2 of Section
IVB).

We have made a in Eq. (1) dimensionless as this seemed the simplest way to ensure consistency.

6) In Section IIA, paragraph 2 (page 3), the authors refer to the
"'Mino time' parameter $\lambda$." While this is still the most
popular nomenclature for this parameter, it was first introduced by
Carter, and a growing number of authors now refer to it as
"Carter-Mino time" or "(Carter-)Mino time" to acknowledge the
contribution by Carter. Therefore the authors may consider referring
to $\lambda$ as "(Carter-)Mino time." I also recommend that, upon
introducing the parameter $\lambda$, that the authors cite the
original Carter and Mino papers, which introduced and popularized this
notation: Carter (1968) (which the authors reference at another point
as Ref [43]), and Mino (2003).

DONE

7) In Section IIA, paragraph 5 (page 3), in the last sentence (after
Eq (2)), the authors state, "We also rescaled the constants of motion
$J$." I recommend that the authors expand upon this statement.
Earlier, the authors define the actions as $J_\beta = (E, L_z, Q,
\mu)$. I would assume that, in general, $J_\beta = (E, L_z, Q, \mu)$
is related to the new $J_\alpha$ in Eq (2) via a non-trivial Jacobian
transformation. If this is the case, it may be worth mentioning that.
I understand that this point is not essential to the work, and may be
why the authors simply refer to it as a "rescaling."

We added a clarification here.

8) In Section IIC, Eq (8) (page 5), I recommend that the authors
define the symbol $\mathbb{E}$. Readers that are not familiar with the
Fisher Information Matrix may not realize that this means the expected
value.

DONE

9) In Section IIIA, in the last paragraph and third to last sentence
(page 6), I recommend changing "...where $\mathcal{T} \sim 1/\eta$" to
"...where the inspiral timescale $\mathcal{T} \sim 1/\eta$". This will
give clear physical meaning to $\mathcal{T}$, which is a newly
introduced symbol that the authors did not previously define.

DONE 

10) In Section IIIB, paragraph 4, last sentence (page 7), the authors
state, "We have checked the validity of this approximation and of the
implemented evolution of phase $\Psi$ in the proximity of the
resonance." I recommend that the authors provide a sentence or two
expanding upon how they validated this approximation.

DONE

11) In Section IVB, paragraph 4, first sentence (page 10), the authors
state, "From Figure (3) we conclude that for resonance coefficients
smaller than $2\times 10^{-5}$ the effects of resonance can be
neglected." I recommend that the authors expand upon how they
determine this cutoff. In other words, can the authors explain at what
point does waveform mismatch not significantly impact data analysis
and parameter estimation?

We changed the limit to $10^{-5}$ and justified this choice using the "indistinguishability criteirion" that appears in the literature. 

12) In Section IVC, paragraph 3, in the second to last sentence (page
11), the authors state, "...the proportion of systems with biases
above 2 sigma is lower, but these proportions still exceed ~85\% and
~27\% respectively." Looking at Figure 3, these ~85% and ~27% values
appear to correspond with 3 sigma biases. I recommend that the authors
double check these numbers.

We checked these numbers. Note that we are talking about the fraction of events exceeding the stated precision, which is one minus what is plotted. 

13) In Appendix A, paragraph 2 (page 14), the authors state, "...it
imposes a limit on the maximum resolvable frequency $f_\mathrm{max} =
1/(2\Delta t)$ [69]." It is unclear how Ref [69] is related to this
statement. If the reference is with respect to the definition of
$f_\mathrm{max}$ then I would recommend that the authors just refer to
the Shannan sampling theorem, and do not need to include this
additional reference. If Ref [69] is supporting another major point,
then I recommend that the authors move [69] closer to the statement it
is supporting.

DONE

14) Lastly, all of the Figures are very difficult to read if the paper
is printed in black and white. I would recommend using different line
types (solid, dashed, dotted) in Figures 1 and 3 in addition to the
different line colors currently used by the authors, and I recommend
that the authors adjust the brightness of the color palettes in
Figures 2, 5, and 6 so that the different colors are distinguishable
when printed on a greyscale. In the Figure captions the authors can
then refer to the line type and color (e.g., "the blue (dot-dashed)
curve depicts..."). This way there is the benefit of color for those
reading the online version (and who are not color blind), while still
making the Figures readable for those who print the paper in black and
white or those who do not distinguish between different types of
colors.

DONE
